Informed Network Coding for Minimum Decoding Delay

Network coding is a highly efficient data dissemination mechanism for wireless networks. Since network coded information can only be recovered after delivering a sufficient number of coded packets, the resulting decoding delay can become problematic for delay-sensitive applications such as real-time media streaming. Motivated by this observation, we consider several algorithms that minimize the decoding delay and analyze their performance by means of simulation. The algorithms differ both in the required information about the state of the neighbors' buffers and in the way this knowledge is used to decide which packets to combine through coding operations. Our results show that a greedy algorithm, whose encodings maximize the number of nodes at which a coded packet is immediately decodable significantly outperforms existing network coding protocols.

==> network_coding.tex <==
\section {Network Coding}
\label{sec:NC}

With network coding, nodes transmit packets coded over multiple
original packets, instead of uncoded data. Coded packets can contain
information from many different data sources.  For coding, sets of
$s$ consecutive bits of a packet are treated as a symbol over the
Galois field $GF(q)$, with $q=2^s$, and an $L$ bits long packet
consists of $L/s$ symbols. Note that coded packets have the same
length as uncoded data packets. Due to its simplicity, usually
\emph{linear} network coding is used, where packets are linear
combinations of the original packets.

For random linear network coding, a packet $Y$ coded over the
original packets $X^1, ..., X^n$ is generated by multiplying each
with a random coding coefficient $g_i$ to obtain $Y=\sum_{i=1}^n g_i
X^i$.  This is done individually for each symbol in the data packet.
It is not necessary to first decode received data in order to create
new coded packets, but the same operations can be applied
recursively to already coded data.

Decoding requires knowledge of the coding coefficients. For
simplicity, assume that a packet contains both the coefficients
$g=(g_1,...,g_n)$ and the encoded data \cite{practical_coding}.
Assume a node has received $(g^1, Y^1),...,(g^m, Y^m)$. Decoding
requires solving the system of equations $\{Y^j=\sum_{i=1}^n g^j_i
X^i\}$ to retrieve the original $X^i$. In case $m \ge n$ and $n$ of
the equations are linearly independent, all data can be recovered.

The special case $GF(2)$ with a field size of $2$ is very appealing
for sensor networks since it only requires addition over a finite
field (which corresponds to a simple {\tt xor}) and no
multiplication. Also the coding coefficients are only a single bit
which reduces overhead and decoding complexity. Different algorithms
are suitable for decoding. Network coding schemes often use Gaussian
elimination to invert the matrix of coding coefficients, but also
methods with lower computational complexity (e.g., message
passing~\cite{Luby02}) can be effectively used in some cases.

To cope with the limited node memory, it is necessary to limit $n$,
the number of packets that can be coded over at the same time.
Packets are grouped into generations~\cite{practical_coding}, and
only packets from the same generation can be combined in the
encoding process.

